Inductive Guided Filter: Real-time Deep Image Matting with Weakly Annotated Masks on Mobile Devices

Recently, significant progress has been achieved in deep image matting. Most of the classical image matting methods are time-consuming and require an ideal trimap which is difficult to attain in practice. A high efficient image matting method based on a weakly annotated mask is in demand for mobile applications. In this paper, we propose a novel method based on Deep Learning and Guided Filter, called Inductive Guided Filter, which can tackle the real-time general image matting task on mobile devices. We design a lightweight hourglass network to parameterize the original Guided Filter method that takes an image and a weakly annotated mask as input. Further, the use of Gabor loss is proposed for training networks for complicated textures in image matting. Moreover, we create an image matting dataset MAT-2793 with a variety of foreground objects. Experimental results demonstrate that our proposed method massively reduces running time with robust accuracy.

==> sections/figures/fail_case.tex <==

\begin{figure}[t]
	\centering
	\begin{subfigure}{0.24\columnwidth}
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/fail_image_1.jpg}}
	\end{subfigure}	
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/fail_alpha_1.png}}
	\end{subfigure}	 
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/fail_image_2.jpg}}
	\end{subfigure}	
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/fail_alpha_2.png}}
	\end{subfigure}	
	
	\caption{Two failed cases in our testing set.}
	\label{fig:fail}
	
\end{figure}

==> sections/figures/fail_case_adobe.tex <==

\begin{figure}[htp]
	\centering
	\begin{subfigure}{0.24\columnwidth}
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_image_1.jpg}}
	\end{subfigure}	
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_trimap_1.png}}
	\end{subfigure}	 
	\begin{subfigure}{0.24\columnwidth}
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_gt_1.png}}
	\end{subfigure}	
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_alpha_1.png}}
	\end{subfigure}	 
	
	
	\centering
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_image_2.jpg}}
		\caption*{Image}
	\end{subfigure}	
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_trimap_2.png}}
		\caption*{Trimap}
	\end{subfigure}	
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_gt_2.png}}
		\caption*{Ground Truth}
	\end{subfigure}	
	\begin{subfigure}{0.24\columnwidth}	
		\centering
		{\includegraphics[width = 1\columnwidth]{figures/data/adobe_failed_alpha_2.png}}
		\caption*{Ours}
	\end{subfigure}	
	
	\caption{Two failed cases in Adobe Composition-1k.}
	\label{fig:fail_adobe}
	
\end{figure}
